Estimating the Decoding Failure Rate of Binary Regular Codes Using Iterative Decoding

Providing closed-form estimates of the decoding failure rate of iterative decoders for low- and moderate-density binary parity-check codes has attracted significant interest in the research community. Recently, interest in this topic has increased due to the use of iterative decoders in post-quantum cryptosystems, where the desired decoding failure rates (DFRs) are less than or equal to $2^{-128}$ and impossible to estimate via Monte Carlo simulations. We propose a new technique that provides accurate DFR estimates for a two-iteration (parallel) bit-flipping decoder that can be used for cryptographic purposes. We estimate the bit-flipping probabilities at the second decoder iteration and the syndrome weight distribution before and after the first iteration as a function of the code parameters and error weight. We validate our results numerically by comparing the modelled and simulated syndrome weights, the incorrectly guessed error bit distribution at the end of the first iteration, and the DFR after two iterations in both the floor and waterfall regimes. Finally, we apply our method to estimate the DFR of the LEDAcrypt cryptographic system, a post-quantum key encapsulation method that employs a two-iteration bit-flipping decoder. We show that the DFR estimate resulting from the chosen code parameters can be improved by a factor larger than $2^{70}$ with respect to previous estimation techniques, when $128$-bit security is required. This allows for a $20$% reduction in public key and ciphertext sizes at no security loss. We note that our results can be applied to the post-quantum cryptosystem known as Bit Flipping Key Encapsulation (BIKE) replacing the current ``BIKE-flip decoder'' with the two-iteration decoder and consequently endowing BIKE with the property of indistinguishability under an adaptive chosen-ciphertext attack (IND-CCA$2$), provably.

==> flipping_probs_extended.tex <==
We now consider the case of the bit under examination being in $\jset{0}{1}$. The expression of $\chi_{\uparrow \mathtt{odd}}(\mathtt{tc},\epsilon_{01})$ is
(changes highlighted in blue):
$$\chi_{\uparrow \mathtt{odd}}(\mathtt{tc},\epsilon_{01})=\sum_{l=1, l\, \text{odd}}^{\tiny
\min(\mathalert{\epsilon_{01}-1}, w-\mathtt{tc}-1)} \frac{ \eta(\mathtt{tc},l)\cdot \zeta(\mathtt{tc},l,\mathalert{\epsilon_{01}-1}) }{ \xi(\mathtt{tc},\mathalert{\epsilon_{01}-1}) },$$

changing from the one when the examined position is in $\jset{0}{0}$ only in 
replacing the occurrences of $\epsilon_{01}$ with $\epsilon_{01}-1$:
indeed, one of the positions $j\in\jset{0}{1}$ involved in the equation being
considered is actually the variable being considered.

The expression of $\chi_{\leftrightarrow \mathtt{odd}}(\mathtt{tc})=$
\noindent
\resizebox{1.05\columnwidth}{!}{
$$
\condprob{\left| \support{h_{i,:}} \cap \jset{1}{1}\right|
\text{is odd}}{\exists a\in \jset{0}{0},h_{i,a}=1,\langle e,h_{i,:}\rangle=\mathtt{tc} },
$$
}
does not change, as the fact that $a$ is in $\jset{0}{1}$ instead of 
$\jset{0}{0}$ does not have any effect on its formulation.

$p_{01|\mathtt{BecomeUnsat}}$ is obtained as (changes highlighted in blue)


$$
\frac{\sum_{\mathtt{tc} = 0, \mathtt{tc}\text{ even}}^{\min(t,w-1)}
\condprob{\flips{\mathtt{tc}}}{\mathalert{\jset{0}{1}}}
\cdot (
\mathalert{1-}
\gamma_{\mathtt{UnsatPostFlips}}(\mathtt{tc},\epsilon_{01},\epsilon_{11})
)
}
{
\sum_{\mathtt{tc} = 0, \mathtt{tc}\text{ even}}^{\min(t,w-1)}
\condprob{\flips{\mathtt{\mathtt{tc}}}}{\mathalert{\jset{0}{1}}}
}
$$
Indeed the two changes from $p_{00|\mathtt{BecomeUnsat}}$ involve the fact 
that the position being considered is in $\jset{0}{1}$ instead of $\jset{0}{0}$
and the fact that the contribution to the parity taking place on the $w-1$ 
positions of the equation excluding the one being considered should be even in order to have an unsatisfied check.
Symmetrically, $p_{01|\mathtt{StayUnsat}}$ is obtained as (changes highlighted in blue)
$$
\frac{\sum_{\mathtt{tc} = 1, \mathtt{tc}\text{ odd}}^{\min(t,w-1)}
\condprob{\flips{\mathtt{tc}}}{\mathalert{\jset{0}{1}}} \cdot
(
\mathalert{1-}
\gamma_{\mathtt{UnsatPostFlips}}
(\mathtt{tc},\epsilon_{01},\epsilon_{11})
)}{
\sum_{\mathtt{tc} = 1, \mathtt{tc}\text{ odd}}^{\min(t,w-1)}
\condprob{\flips{\mathtt{\mathtt{tc}}}}{\mathalert{\jset{0}{1}}}
}.
$$

The probability distribution of the $j$-th upc being valued $a$, given that $j\in\jset{0}{1}$ is (changes w.r.t $\Pr (\mathcal{U}_{j} = a, j\in \jset{0}{0})$ highlighted in blue):
$$\Pr (\mathcal{U}_{j} = a, j\in \jset{0}{1}) =
\begin{cases}
    \frac{\bindist{v}{\punsatz}{a}}{p_{\mathalert{\mathtt{flip}|0}}} & \quad \text{if } x\ \mathalert{\geq}\ \mathtt{th}_{(1)}\\
    0 & \quad \text{otherwise}\\
\end{cases}
$$

Since the expression of $\mu$ does not change, we obtain 
$\pflipzo(\epsilon_{01},\epsilon_{11})$:
$$
\begin{array}{l}
\displaystyle
\pflipzo(\epsilon_{01},\epsilon_{11})=\sum_{\mathalert{a=\mathtt{th}_{(1)}}}^{\mathalert{v}}
\Pr (\mathcal{U}_{j} = a, \mathalert{j\in \jset{0}{1}}) \cdot  \\
\displaystyle
\cdot\left(  \sum_{\mathtt{nsat} = 0}^{v-a} \sum_{
{\tiny \begin{matrix}
\mathtt{nunsat}=\\
\max(0,\mathtt{th}_{(2)}-\mathtt{nsat})
\end{matrix}}
}^{a}  \mu(\mathtt{nsat},\mathtt{nunsat},a,\epsilon_{01},\epsilon_{11})\right)
\end{array}
$$
since we are interested in the probability of performing a flip
at the second iteration (which does not change from the computation
of $\pflipzz$), but the first iteration performed a flip, therefore
the first-iteration upc value $a$ should be above the first iteration
threshold $\mathtt{th}_{(1)}$.

We now move to the case of a bit being in $\jset{1}{0}$. The expression of $\chi_{\uparrow \mathtt{odd}}(\mathtt{tc},\epsilon_{01})$ is:
$$\eta(\mathtt{tc},l) = \bindist{\mathalert{w-\mathtt{tc}}}{\pflipz{\mathtt{OneEqSat}}}{l}$$
$$\chi_{\uparrow \mathtt{odd}}(\mathtt{tc},\epsilon_{01})=\sum_{l=1, l\, \text{odd}}^{\tiny
\min(\epsilon_{01}, \mathalert{w-\mathtt{tc}})} \frac{ \eta(\mathtt{tc},l)\cdot \zeta(\mathtt{tc},l,\epsilon_{01}) }{ \xi(\mathtt{tc},\epsilon_{01}) },$$

where the modified indexed are justified by the fact that the bit we are analyzing is not in the set of initially clear bits, so we do not need to subtract it in the calculation of $\chi_{\uparrow \mathtt{odd}}(\mathtt{tc},\epsilon_{01})$. For the same reason, $\chi_{\leftrightarrow \mathtt{odd}}(\mathtt{tc},\epsilon_{11})$ becomes:
$$\nu(\mathtt{tc},l)=\bindist{\mathalert{\mathtt{tc}-1}}{\pnoflipo{\mathtt{OneEqSat}}}{l}$$
$$\chi_{\leftrightarrow \mathtt{odd}}(\mathtt{tc},\epsilon_{11})= \sum_{l=1, l\, \text{odd}}^{\tiny
\min(\epsilon_{11}, \mathalert{\mathtt{tc}-1})}\frac{ \nu(\mathtt{tc},l)\cdot \lambda(\mathtt{tc},l,\epsilon_{11})
}{\theta(\mathtt{tc},\epsilon_{11})}$$

Where $\mathtt{tc}-1$ is the number of asserted positions in the error vector where a flip may happen. $p_{10|\mathtt{BecomeUnsat}}$ is obtained as

$$
\frac{\sum_{\mathtt{tc} = \mathalert{2}, \mathtt{tc}\text{ even}}^{\min(t,\mathalert{w})}
\condprob{\flips{\mathtt{tc}}}{\mathalert{\jset{1}{0}}}
\cdot
\gamma_{\mathtt{UnsatPostFlips}}(\mathtt{tc},\epsilon_{01},\epsilon_{11})
}
{
\sum_{\mathtt{tc} = \mathalert{2}, \mathtt{tc}\text{ even}}^{\min(t,\mathalert{w})}
\condprob{\flips{\mathtt{\mathtt{tc}}}}{\mathalert{\jset{1}{0}}}
}
$$
substituting $w-1$ with $w$ (since a clear bit in the check is not guaranteed) and $\mathtt{tc} = 0$ with $\mathtt{tc} = 2$ (since an asserted bit is now guaranteed). $p_{10|\mathtt{StayUnsat}}$ is obtained as
$$
\frac{\sum_{\mathtt{tc} = 1, \mathtt{tc}\text{ odd}}^{\min(t,\mathalert{w})}
\condprob{\flips{\mathtt{tc}}}{\mathalert{\jset{1}{0}}} \cdot
\gamma_{\mathtt{UnsatPostFlips}}(\mathtt{tc},\epsilon_{01},\epsilon_{11})}{
\sum_{\mathtt{tc} = 1, \mathtt{tc}\text{ odd}}^{\min(t,\mathalert{w})}
\condprob{\flips{\mathtt{\mathtt{tc}}}}{\mathalert{\jset{1}{0}}}
}.
$$

The probability distribution of the $j$-th upc being valued $a$, given that $j\in\jset{1}{0}$ is (changes w.r.t $\Pr (\mathcal{U}_{j} = a, j\in \jset{0}{0})$ highlighted in blue):
$$\Pr (\mathcal{U}_{j} = a, j\in \jset{1}{0}) =
\begin{cases}
    \frac{\bindist{v}{\mathalert{\punsato}}{a}}{p_{\mathalert{\mathtt{flip}|1}}} & \quad \text{if } x\ \mathalert{\geq}\ \mathtt{th}_{(1)}\\
    0 & \quad \text{otherwise}\\
\end{cases}
$$

Since the expression of $\mu$ does not change, we obtain 
$\pflipoz(\epsilon_{01},\epsilon_{11}):$
$$
\begin{array}{l}
\displaystyle
\pflipoz(\epsilon_{01},\epsilon_{11})=\sum_{\mathalert{a=\mathtt{th}_{(1)}}}^{\mathalert{v}}
\Pr (\mathcal{U}_{j} = a, \mathalert{j\in \jset{1}{0}}) \cdot  \\
\displaystyle
\cdot\left(  \sum_{\mathtt{nsat} = 0}^{v-a} \sum_{
{\tiny \begin{matrix}
\mathtt{nunsat}=\\
\max(0,\mathtt{th}_{(2)}-\mathtt{nsat})
\end{matrix}}
}^{a}  \mu(\mathtt{nsat},\mathtt{nunsat},a,\epsilon_{01},\epsilon_{11})\right)
\end{array}
$$

Finally, we derive the flipping probability of a bit in $\jset{1}{1}$. Switching from $\jset{1}{0}$ to $\jset{1}{1}$ does not change the definition of $\chi_{\uparrow \mathtt{odd}}(\mathtt{tc},\epsilon_{01})$, while $\chi_{\leftrightarrow \mathtt{odd}}(\mathtt{tc},\epsilon_{11})$ becomes:
$$\chi_{\leftrightarrow \mathtt{odd}}(\mathtt{tc},\epsilon_{11})= \sum_{l=1, l\, \text{odd}}^{\tiny
\min(\mathalert{\epsilon_{11}-1}, \mathalert{\mathtt{tc}-1})}\frac{ \nu(\mathtt{tc},l)\cdot \lambda(\mathtt{tc},l,\mathalert{\epsilon_{11}-1})
}{\theta(\mathtt{tc},\mathalert{\epsilon_{11}-1})}$$

where, with the same line of reasoning as the $\jset{0}{1}$ case, we exclude one of the bits in $\jset{1}{1}$ being it the one under consideration. $p_{11|\mathtt{BecomeUnsat}}$ is obtained as

$$
\frac{\sum_{\mathtt{tc} = \mathalert{2}, \mathtt{tc}\text{ even}}^{\min(t,\mathalert{w})}
\condprob{\flips{\mathtt{tc}}}{\mathalert{\jset{1}{1}}}
\cdot
(
\mathalert{1-}
\gamma_{\mathtt{UnsatPostFlips}}(\mathtt{tc},\epsilon_{01},\epsilon_{11})
)}
{
\sum_{\mathtt{tc} = \mathalert{2}, \mathtt{tc}\text{ even}}^{\min(t,\mathalert{w})}
\condprob{\flips{\mathtt{\mathtt{tc}}}}{\mathalert{\jset{1}{1}}}
}
$$
noting that, for the parity check to be unsatisfied, an even number of asserted bits must result from the other $w-1$ bits. $p_{11|\mathtt{StayUnsat}}$ is obtained as
$$
\frac{\sum_{\mathtt{tc} = 1, \mathtt{tc}\text{ odd}}^{\min(t,\mathalert{w})}
\condprob{\flips{\mathtt{tc}}}{\mathalert{\jset{1}{1}}} \cdot
(
\mathalert{1-}
\gamma_{\mathtt{UnsatPostFlips}}(\mathtt{tc},\epsilon_{01},\epsilon_{11})
)}{
\sum_{\mathtt{tc} = 1, \mathtt{tc}\text{ odd}}^{\min(t,\mathalert{w})}
\condprob{\flips{\mathtt{\mathtt{tc}}}}{\mathalert{\jset{1}{1}}}
}.
$$


The probability distribution of the $j$-th upc being valued $a$, given that $j\in\jset{1}{1}$ is (changes w.r.t $\Pr (\mathcal{U}_{j} = a, j\in \jset{0}{0})$ highlighted in blue):
$$\Pr (\mathcal{U}_{j} = a, j\in \jset{1}{1}) =
\begin{cases}
    \frac{\bindist{v}{\mathalert{\punsato}}{a}}{p_{\mathalert{\mathtt{flip}|1}}} & \quad \text{if } x< \mathtt{th}_{(1)}\\
    0 & \quad \text{otherwise}\\
\end{cases}
$$

Since the expression of $\mu$ does not change, we obtain 
$\pflipoo(\epsilon_{01},\epsilon_{11}):$
$$
\begin{array}{l}
\displaystyle
\pflipoo(\epsilon_{01},\epsilon_{11})=\sum_{a=0}^{\mathtt{th}_{(1)}-1}
\Pr (\mathcal{U}_{j} = a, \mathalert{j\in \jset{1}{1}}) \cdot  \\
\displaystyle
\cdot\left(  \sum_{\mathtt{nsat} = 0}^{v-a} \sum_{
{\tiny \begin{matrix}
\mathtt{nunsat}=\\
\max(0,\mathtt{th}_{(2)}-\mathtt{nsat})
\end{matrix}}
}^{a}  \mu(\mathtt{nsat},\mathtt{nunsat},a,\epsilon_{01},\epsilon_{11})\right)
\end{array}
$$
With this analysis, we obtained the probability of performing a flip on each of the four category of bits, in turn allowing us to derive the final DFR estimation as a function of the probability of performing the correct flips during the second iteration of the decoder.
